TribeFlow: Mining & Predicting User Trajectories

Which song will Smith listen to next? Which restaurant will Alice go to tomorrow? Which product will John click next? These applications have in common the prediction of user trajectories that are in a constant state of flux over a hidden network (e.g. website links, geographic location). What users are doing now may be unrelated to what they will be doing in an hour from now. Mindful of these challenges we propose TribeFlow, a method designed to cope with the complex challenges of learning personalized predictive models of non-stationary, transient, and time-heterogeneous user trajectories. TribeFlow is a general method that can perform next product recommendation, next song recommendation, next location prediction, and general arbitrary-length user trajectory prediction without domain-specific knowledge. TribeFlow is more accurate and up to 413x faster than top competitors.

==> applications.tex <==
%!TEX root = paper.tex
In the previous sections we introduced \model. We now turn our attention to our main results when applying \model on different datasets which are described next (Section~\ref{subsec:data}). As for our main results, we begin by discussing how \model compares with Tensor decomposition approaches which exploit a time dimension (Section~\ref{subsec:temptensors}). Next, we present the efficacy of \model when predicting future transitions (Section~\ref{subsec:transitions}). We then discuss how \model extracts semantically meaningful latent representations of our datasets  (Section~\ref{subsec:quali}). Finally, we discuss the scalability of \model (Section~\ref{subsec:scala}).

\subsection{Datasets} \label{subsec:data}

\begin{table*}[t!]
\small
\centering
\caption{Summary of our datasets. For testing, we leave out the last 30\% of transitions on each trace (when ordered by time stamp). The exceptions for this rule are the Yes data which has a pre-defined test set.}
\begin{tabular}{lccccccc}
\toprule
& \Hentity & \SDentity & \# Transitions & \# \Hentity & \# \SDentity & Residence Time & Time Span\\
\cmidrule(r){2-8}
Last.FM-1k          & User & Artist     & 10,132,959 & 992       & 348,156   & Yes & Feb. 2005 to May 2009\\
Last.FM-Groups      & User & Artist     & 86,798,741 & 15,235    & 1,672,735 & Yes & Feb. 2005 to Aug. 2014\\
\cmidrule(r){2-8}
BrightKite          & User & Venue      & 2,034,085  & 37,357    & 1,514,460 & Yes & Apr. 2008 to Oct. 2010 \\
FourSquare          & User & Venue      & 453,429    & 191,061   & 87,345    & Yes & Dec. 2012 to April 2014\\
\cmidrule(r){2-8}
YooChoose           & Session & Product & 19,721,515 & 6,756,575 & 96,094    & Yes & Apr. 2014 to Sept. 2014\\
\cmidrule(r){2-8}
Yes         & Playlist & Song   & 1,542,372  & 11,139    & 75,262    & No & -\\
\bottomrule
\end{tabular}
\label{tab:data}
\end{table*}

We apply \model on various datasets of online and offline information flows that we shall now describe. Our datasets encompass applications of different nature, thus capturing, in a broad sense, various characteristics of user behavior (e.g., the residency time on location based social networks than on music streaming applications). Before continuing, it is important to point our that information flows are largely influenced by the business model of the application from which we gathered our data. For instance, recommendation engines or user interfaces will bias information flows towards certain musical artists, locations or products. Such effects are an integral part of the business model of the application and, more importantly, are difficult to factor out in study such as the one we performed. However, we argue that studying information flows under these effects is a desirable property they are inherent to the application. Moreover, \model can be used in datasets which do not reflect these effects if necessary (e.g., when comparing recommendation engines or user interfaces). 

We now detail our datasets which are summarized in Table~\ref{tab:data}. 

\begin{description}
\item[Last.FM-1k] In our experiments, we explored two different datasets from a popular online music streaming application (Last.FM\footnote{\url{http://last.fm}}). Last.FM is an OSN and online music streaming service that aggregates data from various forms of digital music consumption, ranging from desktop/mobile media players to streaming services (theirs and others)\footnote{Aggregation is done using plugins available on various media players.}. Our first Last.FM dataset was collected in 2009 using a snowball sampling~\cite{Celma2010}. After the snowball sampling, 992 uniformly random users were selected. The dataset contains, for each user, the complete listening history (all plays) from February 2005 to May 2009, the self-declared nationality, age (at the time), and registration date~\cite{Celma2010}. Our first Last.FM dataset, Last.FM-1k, is comprised of 10,132,959 information flows triggered by 992 users to 348,156 musical artists.

\item [Last.FM-Groups] Crawled in August 2014, using the user groups\footnote{Pages in which the user discusses musical artists} feature from Last.FM. This dataset was gathered by manually selecting 17 groups: {\it Active Users}, {\it Music Statistics}, {\it Britney Spears}, {\it The Strokes}, {\it Arctic Monkeys}, {\it Miley Cyrus}, {\it LMFAO}, {\it Katy Perry}, {\it Jay-Z}, {\it Kanye West}, {\it Lana Del Rey}, {\it Snoop Dogg}, {\it Madonna}, {\it Rihanna}, {\it Taylor Swift}, {\it Adelle}, and {\it The Beatles}.  For each group, we crawled the listening history (from February 2005 to August 2014) of a subset of the users (the first users listed in the group)\footnote{We focus on the first (more active) users due to rate limits.}. The total number of crawled users in 15,235. While this dataset has biases towards more active users and pop artists (given our choice of groups), it has over 10 times more users and plays than the Last.FM-1k dataset. Moreover, it allows us to analyze the behavior of fans (based on group membership) of different artists. Finally, this dataset also contains the self-declared age (at the time) of the users and the nationality.

\item[BrightKite] Brightkite was location based social network (LBSN) where users shared their current locations by checking-in the application. Each \hentity in this dataset is a user, whereas the \sdentity are locations the user check-ins to. The dataset is comprised of 37,357 users and 1,514,460 locations. The users account for 2,034,085 check-ins from April 2008 to October 2010. The Brightkite dataset was originally gathered by Cho {\it et al.}~\cite{Cho2011} and is available online\footnote{\url{http://snap.stanford.edu/data/loc-brightkite.html}}.
\item[FourSquare] Our second LBSN dataset was gathered from FourSquare by Sarwt {\it et al.}~\cite{SarwtLARSStar}. Similar to the BrightKite dataset, our FourSquare data captures the check-in behavior of 191,061 users on 87,345 venues. This dataset was gathered focused on users located in the United States Only (although venues are worldwide). Both our BrightKite and the FourSquare datasets contains the residency location (e.g., where users reside) for a subset of users.

\item[YooChoose] We also explore a dataset of user clicks on a large European e-commerce businesses. The YooChoose dataset was recently made available as a part of the 2015 RecSys Challenge\footnote{\url{http://2015.recsyschallenge.com/}}. Here, each user is captured by a session and the information flows capture clicks on different products on the same session. The YooChoose captures roughly 20 million clicks, from 6 million sessions to approximately 20 thousand distinct products. This dataset contains the residency time information for each click. But, given that users are actually represented as sessions, there is a bounder upper-limit on the residency time which is of a few hours (the maximum session time).

\item[Yes] Finally, we also make use of the Yes datasets gathered by~\cite{LME}. This dataset consists of song transitions on popular radios of the United States. We exploit this dataset for a fair comparison with the Latent Markov Embedding approach, since this is the same data exploited by the authors. On this data, there is no explicit user information, but we can use \model by defining a radio play-list (e.g., sequence of songs on a radio show) as an user, and each song as an object. In total this dataset is comprised of 11 thousand playlists, 75 thousand songs from 1.5 million song transitions. It is important to note that the Yes dataset does not contain time-stamped transitions, thus we cannot account for residency times explicitly. Such a fact does not limit the use of \model which can be explored for both datasets with and without residency times. 
\end{description}

Recall that, as described above, our Last.FM, BrightKite and FourSquare datasets contain social-demographic data for the users. The Last.FM datasets describe the users age, nationality and registration date (only on the Last.FM-1k); whereas, the BrightKite and FourSquare datasets describes the latitude and longitude where the users reside (self-declared). We shall exploit this information when the semantic meaningfulness of \model in Section~\ref{subsec:quali}. {\bf Due to limitations in scalability of baseline models, we exploit smaller subsamples of our original datasets when necessary. These subsamples are composed of 30,000 transitions}. Finally, all we split most of the datasets we analyze (the exception is the Yes dataset) in a train set ($D_{train}$) and a test set ($D_{test}$) where: the training set consists of the first 70\% of the trace when ordered by time and the last 30\% are used for testing. The train and test datasets for the Yes data are pre-defined (see~\cite{Chen2012,Chen2013}).

In the next section we begin our discussion on our main results. Initially, we start by showing the fallacy of other Tensor decomposition approaches that rely on representing time as a Tensor dimension. Next, we discuss how \model can be used to predict transitions and show the semantic meaningfulness of latent factors extracted with \model.

\subsection{Predictions with \model} \label{subsec:transitions}

We evaluate \model and baselines using a information retrieval perspective. That is, the ultimate goal of our predictions is to answers questions of the form: {\it what is the most likely object, or destination $d$, that user $u$ will access, after residing in the source $s$ for $\delta$ time?} Given that our datasets are composed of $(d,s,u,\delta)$ quadruples, each question, or {\it query} from the test is defined as the triple $(s,u,\delta)$. Such queries have exactly one correct answer on the test set, $\mathcal{D}_{test}$, which is the destination $d$ of the transition. The task of \model and baseline methods is to generate a ranking of candidate destinations $\tilde{d}$ based on the model learned in the training set $\mathcal{D}_{train}$. Finally, notice that queries can be re-written by dropping one or more elements from the triple $(s,u,\delta)$. That is, if the goal is to capture the most likely destination for any user and for any residency time, we can use just the source $s$ as the query. Thus, we begin our discussion on predictions on showing how \model can rank candidate destinations $\tilde{d}$ for different queries. 

Recall that the output of \model are two matrices ($\Theta$ and $\Psi$) and the residency time distributions of each fast mixing Markov chain $\lambda(\cM)$. From each of these matrices and distributions, it is possible to estimate the probability of a latent space, or fast mixing Markov chain, given an user ($P[ \cM \mid u ] = \Theta(\cM,u)$), the probability of an object $o$ given a fast mixing chain ($P[ o \mid \cM ] = \Psi(o,\cM)$), as well as the probability of a residency time $\delta$ given the chain ($P[\delta \mid \cM] \sim \lambda(\cM)$). Given the graphical model in Figure~\ref{fig:model}, and using the output of \model, we can initially compute the probability of {\it any user} transitioning from $s$ to $\tilde{d}$ after any given residency time as:
\begin{align} \label{eq:general}
P[\tilde{d} \mid s] \propto \sum_{\cM} \Psi(\tilde{d}, \cM) \Psi(s, \cM) n_{\cdot \cM}.
\end{align}

\noindent Here, $n_{\cdot \cM}$ is the number of transitions assigned to latent space $\cM$ and is used as an estimate of $P[\cM]$. We make use of this initial estimation of $P[ \tilde{d} \mid s ]$ for the situations when user information and residency times are not given, such as for the comparing with the LME model (more below), which estimates this same probability using a different approach. Next, we extend the computation above to incorporate users. That is, we can capture the probability that a given user $u$ will transition from $s$ to $\tilde{d}$ as:
\begin{align} \label{eq:user}
P[\tilde{d}\mid s, u] \propto \sum_{\cM} \Psi(\tilde{d}, \cM) \Psi(s, \cM) \Theta(\cM, u)
\end{align}

Finally, we can incorporate the residency time $\delta$ into the model simply by incorporating $\Delta_{\delta \mid z}(\delta,z)$, as shown below:
\begin{align} \label{eq:full}
    P[\tilde{d}\mid s,\delta,u] \propto \sum_{\cM} \Psi(\tilde{d}, \cM) \Psi(s, \cM) \Theta(\cM, u) P[\delta \mid \cM]
\end{align}

As mentioned, each of the equations above can be used in different queries. Eq.~\ref{eq:general} captures the probability of any user going from $s$ to $\tilde{d}$ regardless of the residency time. Eq.~\ref{eq:user} considers a specific user and can thus be exploited for personalized predictions. Finally, Eq.~\ref{eq:full} is used to measure the probability of a user transitioning from $s$ to $\tilde{d}$ after spending $\delta$ time on $s$. 

In order to evaluate the efficacy, we make use of four different metrics. Recall that each metric is evaluated on the test set $\mathcal{D}_{test}$, after the model is learned on the training set $\mathcal{D}_{train}$. For the sake of simplicity, we shall define our efficacy metrics only in terms of $P[d\mid s]$. Our first metric is the {\it predictive likelihood} of the transitions, that is defined as:
\begin{align}
LL(\mathcal{D}_{test}) = \sum_{s,d \in \mathcal{D}_{test}} n_{ds} log(P[d\mid s]).
\end{align}

\noindent In this metric, and all other following, it is important to notice that $d$ is the {\it true} destination of the transition. Thus, models with higher likelihood will assign higher probabilities to the transitions which occur in the test set (higher likelihoods are achieved by better models). Although simple, the interpretability of likelihood values are usually difficult since the metric can range from $-\infty$ to $0$ for discrete probability distributions (such as the ones \model and baselines make use of). %The highest value, $0$, occurs when each transition on the test set has probability of $1$ in the model learned from the training set.

To achieve a higher interpretability, we make use of reciprocal rank based measures to evaluate \model and baselines. The reciprocal rank, $RR$, is the inverse of the position of the real destination $d$ on the ranking of all candidates $\tilde{d}$ in decreasing order. For instance, if three destinations {\it Big Brewery}, {\it Pizza Place}, and {\it Sandwich Shop}, are ranked with probabilities $0.4$, $0.5$, and $0.3$ respectively, and we assume that the {\it true} destination was {\it Big Brewery}, the reciprocal rank has value of $\frac{1}{2}$. We can define $RR$ as:
\begin{align}
    RR(d, s) &= \frac{1.0}{rank(P[d\mid s])}.
\end{align}

\noindent Based on the reciprocal rank we can define two metrics for the whole test set. The mean reciprocal rank, defined as:
\begin{align}
    MRR(\mathcal{D}_{test}) &= \frac{\sum_{s,d \in \mathcal{D}_{test}} RR(d, s)}{|\mathcal{D}_{test}|}.
\end{align}

\noindent Secondly, we can define the mean precision at $k$, which captures the fraction of queries where the correct answer was ranked before or equal to a given cut-off $k$:
\begin{align}
    MeanPrec@k(\mathcal{D}_{test}, k) &= \frac{\sum_{s,d \in \mathcal{D}_{test}} \mathbb{I}_{[RR(d, s) \leq \frac{1}{k}]}}{|\mathcal{D}_{test}|}.
\end{align}
\noindent Where, $\mathbb{I}_{[RR(d, s) \leq \frac{1}{k}]}$ takes value of $1$ when $RR(d, s) \leq \frac{1}{k}$, and value of $0$ otherwise. Given that only one relevant destination exists for each query, $\mathbb{I}_{[RR(d, s) \leq \frac{1}{k}]}$ is equivalent to both the definitions of precision and the recall at cut-off $k$ from information retrieval.

\subsubsection{Baselines}

We now described our baseline models which have been proposed in the literature. We separate our baselines in two-classes: (1) {\it probabilistic low-rank decomposition} model; and, (2) {\it ranking based low-rank decomposition} models. The first class of models create low-rank probability matrices as \model, whereas the second class of models do away with the probabilistic interpretation of the low-rank and focus on rankings only. In this sense, the ranking based models provide a smaller algorithmic complexity (see Table~\ref{tab:salesmat}) at the cost of a lower interpretation of the low-rank space. We begin our description with the probabilist models:


\begin{itemize}
    \item Latent Markov Embedding (LME): We make use of the LME model defined in~\cite{Chen2012,Chen2013}. As we have discussed in our related work, LME will find a low rank decomposition of transitions similar to \model. However, the LME approach is limited since it will not exploit personalized information, residency time or be able to incorporate a Markovian memory to the decomposition (only zero-order transitions are extracted). In all our cases, we train LME using the approach described in~\cite{Chen2013} with the clustering parameter set to 100, as suggested, while varying the number of latent factors. We also exploited the Personalized Variant of LME (PLME)~\cite{Wu2013}. However, due to it's non-parallel nature and huge runtime cost (see Table~\ref{tab:xxx}), PLME is unsuited for our datasets. Moreover, another more scalable baseline we compare with -- Personalized Ranking by Latent Markov Embedding (below) -- has surpassed PLME in terms of efficacy.

    \item Latent Dirichlet Allocation (LDA)~\cite{Blei2006}: We also attempted LDA as transition modeling strategy. Here, we represent each user as the LDA document and each object and the word. LDA will find a latent representation of this matrix which can represent: $P[\cM \mid u]$ and $P[o\mid cM]$. Although the output is similar to \model, LDA will not explicitly capture transitions, residency times or memory. As we shall discuss in our results, the lack of explicit transitions heavily impacts the suitability of LDA the transition prediction task. We can measure $P[d\mid s]$ using LDA as:
        $$P[d\mid s] = \sum_{\cM} P[\cM \mid s] P[d \mid \cM]$$

    \item TransitionMatrix-LDA (TMLDA): We also implemented the TM-LDA~\cite{TMLDA} model. TM-LDA consists of a post-processing of the LDA results to define a low rank Markovian transition matrix. That is, if LDA is trained with $k$ latent factors (the low rank), TM-LDA will create a $(k,k)$ capturing the probability of flowing between these factors. It is imperative to notice that this transition matrix is not between objects. Based on the Bayesian model of LDA, we incorporate this transition matrix to capture transitions between objects as:
        $$P[d\mid s] = \sum_{\cM_d} P[d \mid \cM_d] \sum_{\cM_s} P[\cM_s \mid s] P[\cM_d \mid \cM_s]$$

    \item Gravity Model (GM): Finally, we employ the gravity model which captures the flows of users between two objects. As is the case with LME, GM will not exploit user information, residency time or model memory. Also, GM is limited since it relies on a pre-defined distance function between two objects. Because of this, we only employ the GM model on our location datasets making use of the approximate earth distance\footnote{Distance on the sphere} between two venues. As suggested by various authors~\cite{Quercia,Goods2006,Li2011}, we fit the model using a Poisson regression. By making use of Eq~\ref{eq:gravity}, which defines the gravity model, the Poisson regression fitted using a Generalized Linear Models~\cite{GLM} approach and can be written as: $$log(\mu) = \theta_0 + \theta_1 log(n_s) + \theta_2 log(n_d) - \theta_3 log(dist(d, s))$$ 
    
    Here, $\theta_i$ are model parameters fitted from the training data. $\mu$ is the inverse rate, or expected counts, of the Poisson distribution. If $n_{ds}$ is the number of transitions between $s$ and $d$ on the training set, $log(\mu) = n_{ds}$. To evaluate the GM we make use of the expected number of transitions, $\mu$, of the Poisson distribution to compute the predictive likelihood on the test set. That is\footnote{On this equation, $n_{ds}$ is computed on the test set}, $LL = \sum log(\frac{\mu^{n_{ds}}e^{-\mu}}{n_{ds}!})$. 
\end{itemize}

Secondly, we exploit two state-of-the-art and recent ranking based models:

\begin{itemize}
    \item Factorizing Personalized Markov Chain (FPMC): Rendle {\it et al.}~\cite{Rendle2010} describe a low rank approach to factorize the Markov chains of browsing behavior of individual users. This approach will make use of a Bayesian Belief-Propagation learning algorithm to perform factorizations. As we have discussed in Section~\ref{sec:related}, FPMC is state-of-the-art approach focused on ranking the next destination of users\footnote{\url{http://github.com/flaviovdf/fpmc}}. 

    \item Personalized Ranking by Latent Markov Embedding (PRLME): Very recently the PRLME approach has been proposed to {\it rank} transitions based on low rank decomposition~\cite{Feng2015}. Motivated by the PLME~\cite{Wu2013} model, PRLME is based on optimizing a similar cost function in order to perform the low rank decomposition. However, in order tackle the algorithmic complexity of LME and PLME, the PRLME makes use of a similar learning algorithm as FPMC\footnote{\url{http://github.com/flaviovdf/prme}}.
\end{itemize}

All of our experiments were performed on a cluster of compute nodes with two 10-core Intel Xeon-E5 processors (20 cores per node) and 256 GB of memory. Even though \model is implemented using MPI, on most of our experiments we exploit the 20 cores of a single node. On the cases where we performed the learning on more than one node, the inter-node communication exploits a 40 Gbps Ethernet connection between nodes. In the next subsections we present our prediction results.

\subsubsection{Comparison with Probabilistic Models} 

\begin{figure}[t]
    \centering
    \subfigure[Predictive LL]{\includegraphics[scale=.95]{figs/ll_lme.pdf}}
    \subfigure[Runtime]{\includegraphics[scale=.95]{figs/speed_lme.pdf}}
    \caption{Comparing \model with LME~\cite{Chen2012,Chen2013}.}
    \label{fig:lme_comp}
\end{figure}


{\bf \model vs LME} We begin our discussion by comparing \model with Latent Markov Embedding. In Figure~\ref{fig:lme_comp}(a) we show the average predictive likelihood of \model and of LME. We present our results when decomposing user transitions in $10$ and $50$ latent factors. More importantly, results are only shown for the Yes dataset and the FourSquare dataset. This is because LME is unable to handle all of our other datasets either due scalability issue, which we shall discuss shortly, and also due to code limitations (e.g., the LME code available online\footnote{URL} cannot handle playlists, or users, with over 10,000 transitions a common setting in online data)\footnote{We also found that the code would randomly crash even on small datasets.}. Due to these limitations, we are also unable to report results on the FourSquare dataset with 50 latent factors due to crashes in the authors original source code.

Each column in Figure~\ref{fig:lme_comp}(a) represents the average predictive likelihood of a model. CF stands for \model, whereas CF-Mem is \model when trained with $m=2$, that is a one-order Markov chain. From Figure~\ref{fig:lme_comp}(a) we can see that, we can initially notice that \model achieves better results than LME on the Yes datasets. LME achieves predictive likelihood values of -6.74 and -6.72 when using 10 and 50 latent factors respectively. \model achieves -6.65 and -6.55 on these very same settings. When adding a memory, we can notice an improvement to \model. In this cases, results are of -6.39 and -6.29. Overall, on the Yes dataset, we can state that both models achieve similar results, with \model being slightly better (up to 3\% improvement). Nevertheless, when we look into the FourSquare dataset, we can see that LME achieves a score of -7.17, whereas \model can achieve a score of -5.94 with memory, thus achieving a 17\% gain. Finally, as we have discussed LME is unable to handle our FourSquare dataset with 50 latent factors. In this setting, \model achieved a likelihood of -5.45, and is this 23\% more accurate than the best attempt of decomposing the transitions (with 10 factors) of \model. 

We further emphasize the limitations of the LME approach by showing in Figure~\ref{fig:lme_comp}(b) the execution time of \model and LME. From this figure, it is clear that while LME requires at least 7 hours (25,755 seconds) to process the Yes and FourSquare datasets with 10 latent factors, \model can achieve better results, as discussed, in under 8 minutes. The gains in runtime can reach 400x, as is the case in FourSquare dataset in particular where \model executes in under 51 seconds. Thus, even if the LME source were able to handle our larger datasets (with over 80 million transitions), given the algorithmic complexity of model, we estimate that it would take months to analyze our datasets with this approach.

{\bf \model vs LDA Approaches}


\begin{table}[t!]
\scriptsize
\centering
\caption{Comparing \model with the Gravity Model. \model was trained with $k=10$}
\begin{tabular}{lccc}
\toprule
& GM & CF & Gain\\ 
\cmidrule(r){2-4}
FSq.   & -17.28 & {\bf -6.18}  & {\bf 63\%} \\
BKite. & -19.73 & {\bf -10.61} & {\bf 91\%} \\
\bottomrule
\end{tabular}
\label{tab:gmcompare}
\end{table}

{\bf \model vs Gravity Models} We now turn our attention to the specialized Gravity Model. As explained, a Gravity Models are suited for geo-located datasets. Thus, in Table~\ref{fig:gmcompare} we compare the predictive likelihood of \model with the Gravity Model (GM) approach on our FourSquare and Brightkite data. Here, we make use of \model without any residency time resolution with 10 latent factors. From the table, we can see that even with this simple 10 latent factors setting, \model clearly out-performs the Gravity Model approach, with gains reaching up to 91\% on the BrightKite dataset. In more details, \model achieved a predictive likelihood of -10.61, whereas the GM approach achieved -19.73. The gain on the BrightKite dataset was of 63\%. 

%Before continuing to other baselines, it is important to recall that Gravity Models are usually employed to answer questions of the form: {\it given that $n_s$ individuals are in location $s$ and $n_d$ individuals are in location $d$, what is the flow of individuals, or goods, between $s\Rightarrow d$ ($n_{ds}$)}. We can answer questions of this form using GM since it is a regression based approach and $n_s$ and $n_d$ are the covariates. Using \model, we can answer this very same question simply by multiplying $n_s$ by $P[d \mid s]$ ($\tilde{n_{ds}} = n_s P[d \mid s]$). In Figure~\ref{fig:gmpred}(a-d) we show the predictions performed both the GM model as well as the \model model. Figures~\ref{fig:gmpred}(a-b) show results for the FourSquare dataset, whereas Figures~\ref{fig:gmpred}(c-d) shows the same results for the BrightKite data. The $x$ axis of each plot is the predicted flow $\tilde{n_{ds}}$ between $s$ and $d$, whereas the $y$ axis presents the actual flow $n_{ds}$. In each plot we also show the $R^{2}$ score and the mean squared error (MSE)\footnote{$MSE = \sum_{d,s \in D_{test}} \frac{(\tilde{n_{ds}} - n_{ds})^{2}}{|D_{test}|}$}.

\subsubsection{Comparison with Ranking Models}

\begin{figure*}[t]
    \centering
    \subfigure[LastFM-1k]{\includegraphics[scale=1]{figs/lastfm_ocelma.pdf}}
    \subfigure[LastFM-Groups]{\includegraphics[scale=1]{figs/lastfm_our.pdf}}
    \subfigure[Brightkite]{\includegraphics[scale=1]{figs/brightkite.pdf}}
    \subfigure[FourSquare]{\includegraphics[scale=1]{figs/four_sq.pdf}}
    \subfigure[YooChoose]{\includegraphics[scale=1]{figs/yoochoose.pdf}}
    \caption{Comparing the Dynamic \model.}
    \label{fig:rrdyn}
\end{figure*}

We now focus our comparison of \model with other ranking approaches. Before continuing, we show how our dynamic learning algorithm improves the efficacy of \model.

\begin{itemize}
    \item Figure~\ref{fig:rrdyn} will show how our dynamic fitting strategy helps
    \item Improvements on the reciprocal rank
\end{itemize}

\begin{table*}[t!]
\scriptsize
\centering
\caption{Comparing \model with other ranking approaches (small dataset 30k, need to look into scalability of baselines)}
\begin{tabular}{llcccccccccc}
\toprule
& & 2 & 4 & 8 & 16 & 32 & 64 & 128 & 256 & 512 & 1024\\
\cmidrule(r){2-12}
\multirow{3}{*}{\begin{sideways}BKite\end{sideways}} & cfdyn  (our)    & 0.04363 &0.08029 &0.07782 &0.09804 &0.14254 &0.21463 &0.27152 &0.36945 &0.4277  & {\bf 0.57734} \\
& fpmc (www2010)  & 0.00021 &0.00021 &0.00021 &0.00021 &0.00021 &0.00021 &0.00021 &0.00021 &0.00021 &0.00021 \\
& prme (jcai2015) & 0.14153 &0.24954 &0.45724 &0.47611 &0.46597 &0.46224 &0.47254 &0.47956 &0.47513 &0.46787 \\
\cmidrule(r){2-12}
\multirow{3}{*}{\begin{sideways}FourSq\end{sideways}} &cfdyn  (our)    &   0.12315 &   0.17665 &   0.1631  &   0.14487 &   0.14821 &   0.17345 &   0.17955 &   0.17374 &   0.16461 &   0.1473 \\
&fpmc (www2010)  &   0.00023 &   0.00023 &   0.00023 &   0.00023 &   0.00023 &   0.00023 &   0.00023 &   0.00023 &   0.00023 &   0.00023\\
&prme (jcai2015) &   0.05032 &   0.05497 &   0.05878 &   0.06306 &   0.07117 &   0.07843 &   0.07389 &   0.08256 &   0.07077 &   0.07327\\
\cmidrule(r){2-12}
\multirow{3}{*}{\begin{sideways}LFM-1k\end{sideways}} &cfdyn  (our)    &   0.10247 &   0.12158 &   0.12555 &   0.1446  &   0.16317 &   0.15949 &   0.15941 &   0.16668 &   0.16373 &   0.16735\\
&fpmc (www2010)  &   0.00048 &   0.00048 &   0.00048 &   0.00048 &   0.00048 &   0.00048 &   0.00048 &   0.00048 &   0.00048 &   0.00048\\
&prme (jcai2015) &   0.07571 &   0.10035 &   0.1169  &   0.12307 &   0.11874 &   0.12018 &   0.12169 &   0.11349 &   0.11605 &   0.10354\\
\cmidrule(r){2-12}
\multirow{3}{*}{\begin{sideways}LFM-G\end{sideways}} &cfdyn  (our)    &   0.08703 &   0.14832 &   0.14764 &   0.16054 &   0.18351 &   0.19536 &   0.17841 &   0.1867  &   0.1904  &   0.18301\\
&fpmc (www2010)  &   0.00043 &   0.00043 &   0.00043 &   0.00043 &   0.00043 &   0.00043 &   0.00043 &   0.00043 &   0.00043 &   0.00043\\
&prme (jcai2015) &   0.09876 &   0.10466 &   0.11643 &   0.11769 &   0.12285 &   0.11765 &   0.12502 &   0.11744 &   0.10837 &   0.10861\\
\cmidrule(r){2-12}
\multirow{3}{*}{\begin{sideways}Yoo\end{sideways}} &cfdyn  (our)    &   0.06433 &   0.11455 &   0.1189  &   0.13346 &   0.16998 &   0.17676 &   0.19067 &   0.21039 &   0.2219  &   0.25591\\
&fpmc (www2010)  &   0.00037 &   0.00037 &   0.00037 &   0.00037 &   0.00037 &   0.00037 &   0.00037 &   0.00037 &   0.00037 &   0.00037\\
&prme (jcai2015) &   0.0804  &   0.06106 &   0.07047 &   0.08125 &   0.09398 &   0.09236 &   0.09428 &   0.09299 &   0.09525 &   0.09153\\
\bottomrule
\end{tabular}
\label{tab:mrrbaselines}
\end{table*}




\subsection{Exploratory Analysis with \model}

\subsubsection*{Artist to Artist Transitions}

\begin{table*}[t]
\scriptsize
\centering
\caption{BECOMES WORD CLOUD. Example Genes Extracted From the Last.FM-Groups Tartest: top sources and destination artists, and demographics of top-50 users. Sources, destinations, and users are sorted based on the probabilities defined by \model in Section~\ref{sec:model}. (BR = Brazil, US = USA, NL = Netherlands, DE = Germany, PL = Poland, FI = Finland) . Ages are 25th, median and 75th percentiles}
\begin{tabular}{lcccccccc}
%    \toprule
    &\multicolumn{2}{c}{Gene=18 (BR/US pop artists)} & \multicolumn{2}{c}{Gene=20 (metal artists) } & \multicolumn{2}{c}{Gene=23 (electronic dance artists)} & \multicolumn{2}{c}{Gene=39 (Pop artists)}\\
    &Sources & Destinations & Sources & Destinations & Sources & Destinations & Sources & Destinations \\
    \cmidrule(r){1-3}    \cmidrule(r){4-5}     \cmidrule(r){6-7} \cmidrule(r){8-9}
\multirow{7}{0pt}{\begin{sideways}Artists\end{sideways}} &
Britney Spears & Britney Spears         & Nightwish &  Nightwish                  & Daft Punk & Daft Punk & Britney Spears & Britney Spears \\
               &Wanessa & Wanessa                       & Within Temptation & Within Temptation  & David Guetta & Deadmau5 & Madonna & Christina Aguilera\\
               &Christina Aguilera & Christina Aguilera & Evanescence & Evanescence              & Skrillex & Skrillex &Christina Aguilera & Madonna\\
               &t.A.T.u. & t.A.T.u.                     & Epica & Epica                          & Deadmau5 & David Guetta &Rihanna & Rihanna\\
               &Katy Perry & Katy Perry                 & Korn &   Korn                          & The Prodigy & The Prodigy & Lady Gaga&Lady Gaga\\
               &Claudia Leitte & Claudia Leitte         & Disturbed & Disturbed                  &Tiesto & Pendulum & Katy Perry & Katy Perry\\
               &Lady Gaga & Pitty                       & Marilyn Manson &  Marilyn Manson       & Pendulum & Tiesto & Kesha & Kesha\\
    \cmidrule(r){1-3}    \cmidrule(r){4-5}     \cmidrule(r){6-7} \cmidrule(r){8-9}
\multirow{2}{0pt}{\begin{sideways}Users\end{sideways}} 
    & \multicolumn{2}{c}{BR=98\%, NL=2\%}      &  \multicolumn{2}{c}{DE = 18\%,  PL = 16\%, US = 12\%} & \multicolumn{2}{c}{US = 18\%, BR = 10\%,} \\
    & &  &   \multicolumn{2}{c}{ FI = 8\%, UK = 6\%}  & \multicolumn{2}{c}{PL = 10\%, UK = 10\%} & \multicolumn{2}{c}{BR=78\%, US=10\%, PL=5\%}  \\
    &\multicolumn{2}{c}{Age: 19; 21;24 (min 16, max 34)}  & \multicolumn{2}{c}{Age: 21; 24; 29 (min 13; max 60)} & \multicolumn{2}{c}{Age: 20; 22; 25 (min 17; max 33)} & \multicolumn{2}{c}{Age: 19; 22; 25 (min 16; max 41)}\\
 %   \bottomrule
\end{tabular}
\label{tab:genes}
\end{table*}

\subsubsection*{Geolocated Transitions}

\subsection{Lack of Stationarity \& Ergodicity} \label{subsec:temptensors}

One key aspect of \model is the representation of data  based on a user-object-object tensor. Most approaches that mine user behavior over time represent tensors with an explicit as one coordinate. Such methods are are designed to capture synchronous behavior. As is expected from online data, and we have described in our datasets, real-world data will span multiple years covering the preferences of a diverse set of users. In order to exemplify the asynchrony effect, looked into the registration date of different users in our Last.FM-1k dataset. We found that, on average, a new user will arrive on the application every other day (2 days between arrivals), with 50\% of the user registrations happening in a day or less. Given that, new users arrive at the application at different times, it is highly unlikely that users with the same taste will have synchronous behavior, as we further discuss next. 

We can measure the asynchrony of users by looking into the dispersion of the unique users that access an object. The arrival of new user at a certain time can be used as a proxy the initial interest of the user to an object. Complementary, the last access a user issued to an object will show, to a certain extent, the abandonment or loss of interest of the users to the certain object\footnote{It is impossible to say for sure if a user lost interest in an object, but we can use the last access as a proxy for loss of interest in the span of our datasets}.

\begin{itemize}
    \item {\bf TODO:} we need a test for synchrony
\end{itemize}

To provide further evidence in support of our  method, we show that unlike temporal tensor approaches, our model is able to more accurately recover the inherent preferences of each user. Since explicit user preferences are not available in our datasets, we  built a synthetic dataset with 50 users, split into 5 homogeneous groups with pre-defined distributions of preferences which are determined by different object popularity distributions (each distribution is a preference)\footnote{We modeled  the object popularity of each group using a different Lognormal distributions~\cite{Figueiredo2014}.}. For each user,  we produced a sequence of transitions with exponentially distributed residency times. Starting from a random object, for each transition, we sampled a destination object from the preference distribution of the user group with probability 0.99. We sampled the destination from a different distribution with probability 0.01 (to introduce some noise).  We simulated a total of 5 days, and each user performs 100 plays per day.  We simulated users joining the system at different times by starting their sequences of plays at different days (1 or 2 days apart).
 
\begin{figure}[t]
    \centering
    \includegraphics[scale=.75]{figs/trimine_compare.pdf}
    \caption{Comparison with Temporal Decomposition.}
    \label{fig:trimine}
\end{figure}

We applied  our model and a  temporal decomposition method~\cite{Matsubara2012a} on our synthetic dataset, aiming at recovering the groups of musical preferences.  Figure~\ref{fig:trimine}  plots the matrices $\mathbf{\Theta}$, which captures the user preferences on the latent space, produced by both methods and the ground truth
 (i.e, user ids  $[0,10)$ in group 0, $[10, 19 )$ in group 1, etc). Clearly, our method is able to recover the different user groups (blocks in the matrix), despite the asynchronous behavior of users within each group. In contrast,  the temporal decomposition fails to do so,  mixing users of  different groups together.

In this section we have discussed the issues of ergodicity faced by Tensor decomposition approaches. We show how \model can dead with these issues, being thus more suitable for analyzing online user behavior. In the next section we shall look into how \model can be used to perform predictions. This shall be done by comparing \model to baseline approaches when predict the next transition of an user.



\subsection{Scalability of \model}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


